OneGen: Efficient One-Pass Unified Generation and Retrieval for LLMs

Despite the recent advancements in Large Language Models (LLMs), which have significantly enhanced the generative capabilities for various NLP tasks, LLMs still face limitations in directly handling retrieval tasks. However, many practical applications demand the seamless integration of both retrieval and generation. This paper introduces a novel and efficient One-pass Generation and retrieval framework (OneGen), designed to improve LLMs' performance on tasks that require both generation and retrieval. The proposed framework bridges the traditionally separate training approaches for generation and retrieval by incorporating retrieval tokens generated autoregressively. This enables a single LLM to handle both tasks simultaneously in a unified forward pass. We conduct experiments on two distinct types of composite tasks, RAG and Entity Linking, to validate the pluggability, effectiveness, and efficiency of OneGen in training and inference. Furthermore, our results show that integrating generation and retrieval within the same context preserves the generative capabilities of LLMs while improving retrieval performance. To the best of our knowledge, OneGen is the first to enable LLMs to conduct vector retrieval during the generation.

==> idea.tex <==

\section{Introduction}
% intro + abs: 2

\section{Preliminaries and Related Work}
% 1
% 1. 主要目的是为了引入任务。定义后可以对现有的工作进行一个unify，主要就是对任务进行一个统一，且我们的重点是复合任务
% 1.1 也可以谈一下和现有工作的区别，根本原因是query的两次编码，定义query的两次编码为pipeline。只不过有些将检索器和生成器联合优化，有些没有。还有一个例外就是gritlm，一个模型，但是本质上query仍然编码两次。
% 芃晨写的挺精炼，挺好的
% 到底要不要区分任务，R->G
% 2. 讲一下统一在一个上下文的优点
% \subsection{Unified Task Definition}

% \subsection{Motivation}

\section{Method}
% 方法部分需要按照审稿人的建议，再看看，是从token的角度去讲，还是换个别的角度
% 1.5
\subsection{A case study in inference}

\section{Experiment}
% 3.5~4
\subsection{Exprimental Settings}
\textbf{}

\section{Related Work}
\section{Conclusion and Future Work}
% 0.5


% 2, 1, 1.5, 4, 0.5 = 9

% 2, 1, 2, 3.5, 0.5 = 9

\appendix
\section{Relation to Prior Work on LLM instruction Tuning}

\section{Related Work}

\section{Broader application}

==> sections/related_work.tex <==
\section{Related Work}
We refer to Appendix~\ref{app:priorwork} for extensively discussion on relation to prior work on generative and representative instruction tuning, which is the most relevant to our training framework. We refer to   \S~\ref{preliminaries:RGtask}  for prior work on single-time retrieval augmented generation, and   \S~\ref{preliminaries:GRtask}  for prior work on entity linking. Our method is a generic framework that unifies generation and retrieval task and applicable to both.

\subsection{Derivative of RAG}
We notice an increasing number of work related to composite generation and retrieval task. For example, Self-rag\cite{asai2023selfrag} trains an arbitrary LM to generate text with reflection tokens to enhances an LM’s quality and factuality through retrieval and self-reflection. However, the purpose of reflection tokens are completely different from our retrieval tokens, and they still use a separate retriever. Active RAG\cite{jiang2023active} involves multiple retrieval during generation to facilitate continually gathering information throughout the generation. Also, a generation-then-retrieval framework is propose for KBQA, where logic form is generated with fine-tuned LLMs, then retrieving and replacing entities and relations with an unsupervised retrieval method\cite{luo2024chatkbqa}. However, \ours~is a pluggable framework which can be applied on top of these methods.

==> tables/avg_ed.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{ccccc}
\toprule
    & ReFinED & \begin{tabular}[c]{@{}c@{}}ChatEL \\ (GPT-4)\end{tabular} & \begin{tabular}[c]{@{}c@{}}EntGPT-I \\ (GPT-3.5)\end{tabular} & \begin{tabular}[c]{@{}c@{}}OneGen \\ (Llama2$_{\texttt{7B}}$)\end{tabular} \\ \midrule
AVG. & 77.6    & 80.4           & {\underline{84.3}}         & \textbf{86.5}      \\ \bottomrule
\end{tabular}
% \caption{Performance of various models on Entity Disambiguation, showing average F1 scores across nine datasets. 
% \zjt{Detailed results are in Table~\ref{} in Appendix.}}
\caption{
Impact of \ours ~on retrieval capabilities assessed through the Entity Disambiguation task, presenting average F1 scores across nine datasets.
% \zjt{
Detailed results are in Table~\ref{table:app:exp:gr:ed} in Appendix.
% }
}
\label{table:exp:impact:gr:ed}
\end{table}

==> tables/avg_md.tex <==
% \begin{table}[]
% \centering
% \small
% \begin{tabular}{lccc}
% % \toprule
% % \textbf{Method}           & \textbf{AVG.}  \\ \midrule
% % ReFinED          & 72.7 \\ \midrule
% % Llama2$_{\texttt{7B}}$ SFT    & 71.1 \\
% % Llama2$_{\texttt{7B}}$ \ours & 71.5 \\ \bottomrule
% \toprule
% Method & ReFinED & Llama2$_{\texttt{7B}}$ SFT & Llama2$_{\texttt{7B}}$ \ours \\ \midrule
% AVG.   & 72.7    & 71.1   & 71.5   \\ \bottomrule
% \end{tabular}
% \vspace{-1mm}
% \caption{Impact of \ours ~on generation capabilities assessed through the Mention Detection task, presenting average F1 scores across seven datasets.}
% \label{table:exp:impact:gr:md}
% \vspace{-1.5mm}
% \end{table}

% \begin{table}[]
% \vspace{-1mm}
\begin{wraptable}{r}{4cm}
\centering
\small
\begin{tabular}{ll}
\toprule
\textbf{Method} & \textbf{AVG.} \\ \midrule
ReFinED & 72.7 \\
Llama2$_{\texttt{7B}}$ (SFT) & 71.1 \\
Llama2$_{\texttt{7B}}$~(\ours) & 71.5 \\ \bottomrule
\end{tabular}
% \end{table}
\vspace{-1mm}
\caption{Impact of \ours ~on generation capabilities assessed through the Mention Detection task, presenting average F1 scores across seven datasets.}
\label{table:exp:impact:gr:md}
\vspace{-1.5mm}
\end{wraptable}

==> tables/cot_rag.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{wraptable}{r}{8cm}
% 这里还可以把检索器也放上去
\begin{table}[]
% \centering
\small
\scalebox{0.75}{
\begin{tabular}{clcccclcc}
\toprule
\multicolumn{1}{l}{} & & \multicolumn{4}{c}{\textbf{End-to-End Generation}} & & \multicolumn{2}{c}{\textbf{End-to-End Retrieval}} \\ \cmidrule{3-6} \cmidrule{8-9} 
\multicolumn{1}{l}{} & & \multicolumn{2}{c}{HotpotQA} & \multicolumn{2}{c}{2WIKI} & & HotpotQA & 2WIKI \\
\multicolumn{1}{l}{} & & EM & F1 & EM & F1 & & Recall@1 & Recall@1 \\ \midrule
\multirow{2}{*}{Llama2-7B} & \multicolumn{1}{l|}{Baseline} & 52.83 & 65.64 & 70.02 & 74.35 & \multicolumn{1}{l|}{} & 73.76 & 68.75 \\
 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}OneGen} & \textbf{\cellcolor[HTML]{EFEFEF}54.82} & \textbf{\cellcolor[HTML]{EFEFEF}67.93} & \textbf{\cellcolor[HTML]{EFEFEF}75.02} & \textbf{\cellcolor[HTML]{EFEFEF}78.86} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}{}} & \textbf{\cellcolor[HTML]{EFEFEF}{75.90}} & \textbf{\cellcolor[HTML]{EFEFEF}{69.79}} \\ \midrule
\multirow{2}{*}{Llama3.1-7B} & \multicolumn{1}{l|}{Baseline} & 53.72 & 66.46 & 70.92 & 75.29 & \multicolumn{1}{l|}{} & 69.79 & 66.80 \\
 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}OneGen} & \textbf{\cellcolor[HTML]{EFEFEF}55.38} & \textbf{\cellcolor[HTML]{EFEFEF}68.35} & \textbf{\cellcolor[HTML]{EFEFEF}75.88} & \textbf{\cellcolor[HTML]{EFEFEF}79.60} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}{}} & \textbf{\cellcolor[HTML]{EFEFEF}{72.55}} & \textbf{\cellcolor[HTML]{EFEFEF}{68.98}} \\ \midrule
\multirow{2}{*}{Qwen2-1.5B} & \multicolumn{1}{l|}{Baseline} & 48.55 & \textbf{61.02} & 68.32 & 72.66 & \multicolumn{1}{l|}{} & 72.41 & 67.70 \\
 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}OneGen} & \textbf{\cellcolor[HTML]{EFEFEF}48.75} & \cellcolor[HTML]{EFEFEF}{60.98} & \textbf{\cellcolor[HTML]{EFEFEF}73.84} & \textbf{\cellcolor[HTML]{EFEFEF}77.44} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}{}} & \textbf{\cellcolor[HTML]{EFEFEF}{72.70}} & \textbf{\cellcolor[HTML]{EFEFEF}{69.27}} \\ \midrule
\multirow{2}{*}{Qwen2-7B} & \multicolumn{1}{l|}{Baseline} & 53.32 & 66.22 & 70.80 & 74.86 & \multicolumn{1}{l|}{} & 74.15 & 69.01 \\
 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}OneGen} & \textbf{\cellcolor[HTML]{EFEFEF}55.12} & \textbf{\cellcolor[HTML]{EFEFEF}67.60} & \textbf{\cellcolor[HTML]{EFEFEF}76.17} & \textbf{\cellcolor[HTML]{EFEFEF}79.82} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}{}} & \textbf{\cellcolor[HTML]{EFEFEF}{75.68}} & \textbf{\cellcolor[HTML]{EFEFEF}{69.96}} \\ \bottomrule
\end{tabular}
}
\vspace{-1mm}
\caption{
Performance comparison across different datasets using different LLMs.
The end-to-end generation evaluates the model's output.
% 这里有点问题，因为这个的检索是联合的评估
The end-to-end evaluates the 
}
\label{table:exp_cot_rag}
\vspace{-1.5mm}
\end{table}
% \end{wraptable}

==> tables/loss_function.tex <==
% loss
% deploy memory
% Candidate
% Generation and Retrieval

% \begin{wraptable}{r}{4.8cm}
% \centering
% \small
% \scalebox{0.8}{
% \begin{tabular}{lccc}
% \toprule
%         & EL (7)            & ED (9)           & MD (7)            \\ \midrule
% BPR     & \textbf{64.0} & \textbf{86.5} & \textbf{71.5} \\
% InfoNCE & 61.8          & 84.5          & 70.7          \\ \bottomrule
% \end{tabular}
% }
% \caption{Ablation study results of $\mathcal{L}_r$ on EL, ED, and Mention Detection (MD) tasks.
% The table reports average F1 scores for each task.}
% \label{table:exp:ablation:gr:loss}
% \end{wraptable}

\begin{table}[]
\scalebox{1}{
\begin{tabular}{lcc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task}}} & \multicolumn{2}{c}{\textbf{Loss Function ($\mathcal{L}_r$})} \\ \cmidrule{2-3} 
\multicolumn{1}{c}{}                               & InfoNCE           & BPR                    \\ \midrule
EL(7)                                              & 61.8              & \textbf{64.0}          \\
ED(9)                                              & 84.5              & \textbf{86.5}          \\
MD(7)                                              & 70.7              & \textbf{71.5}          \\ \bottomrule
\end{tabular}
}
\caption{Ablation study results of $\mathcal{L}_r$ on EL, ED, and Mention Detection (MD) tasks.
The table reports average F1 scores for each task.}
\label{table:exp:ablation:gr:loss}
\end{table}

==> tables/table_merge2.tex <==
\begin{figure}[t]
\begin{minipage}{0.66\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/ablation_lambda.pdf} 
    \caption{Performance comparison across different datasets using different LLMs. The end-to-end generation evaluates the model's output.}
    \label{fig:exp:ablation:rg:lambda}
\end{minipage}\hfill
\begin{minipage}{0.32\textwidth} 
    \centering
    \small
    \begin{tabular}{ll}
    \toprule
    \textbf{Method} & \textbf{AVG.} \\ \midrule
    ReFinED & 72.7 \\
    Llama2$_{\texttt{7B}}$ (SFT) & 71.1 \\
    Llama2$_{\texttt{7B}}$~(\ours) & 71.5 \\ \bottomrule
    \end{tabular}
    \captionof{table}{Impact of \ours ~on generation capabilities assessed through the Mention Detection task, presenting average F1 scores across seven datasets.}
    \label{table:exp:impact:gr:md}
\end{minipage}
\vspace{-2mm}
\end{figure}


==> tables/table_merge3.tex <==
% \begin{figure}[t]
% \begin{minipage}{0.33\textwidth}
%     \centering
%     \small
%     \begin{tabular}{ll}
%     \toprule
%     \textbf{Method} & \textbf{AVG.} \\ \midrule
%     ReFinED & 72.7 \\
%     Llama2$_{\texttt{7B}}$ (SFT) & 71.1 \\
%     Llama2$_{\texttt{7B}}$~(\ours) & 71.5 \\ \bottomrule
%     \end{tabular}
%     % \end{table}
%     \vspace{-1mm}
%     \captionof{table}{Impact of \ours ~on generation capabilities assessed through the Mention Detection task, presenting average F1 scores across seven datasets.}
%     \label{table:exp:impact:gr:md}
% \end{minipage}\hfill
% \begin{minipage}{0.33\textwidth} 
%     \centering
%     \small
%     \scalebox{1.0}{
%     \begin{tabular}{lr}
%     \toprule
%     \textbf{Method} & \textbf{AVG.}                \\ \midrule
%     ReFinED & 77.6 \\
%     ChatEL(GPT-4) & 80.4 \\
%     EntGPT-I(GPT-3.5) & {\underline{84.3}} \\
%     \ours & \textbf{86.5} \\ \bottomrule
%     \end{tabular}
%     }
%     \captionof{table}{Impact of \ours~on retrieval capabilities assessed through the ED task, presenting average F1 score across nine datasets. Detailed results are in Table in Appendix.}
%     \label{table:exp:impact:gr:md}
% \end{minipage}
% \vspace{-2mm}
% \end{figure}
\begin{wrapfigure}{r}{7.3cm} % "l" 表示表格在左边，适当调整表格宽度
\centering
\begin{minipage}{0.25\textwidth}
    \centering
    \small
    \scalebox{0.8}{
    \begin{tabular}{ll}
    \toprule
    \textbf{Method} & \textbf{AVG.} \\ \midrule
    ReFinED & 72.7 \\
    Llama2$_{\texttt{7B}}$ (SFT) & 71.1 \\
    Llama2$_{\texttt{7B}}$~(\ours) & 71.5 \\ \bottomrule
    \end{tabular}
    }
    \vspace{-1mm}
    \caption{Impact of \ours~on generation capabilities assessed through the Mention Detection task, presenting average F1 scores across seven datasets.}
    \label{table:exp:impact:gr:md}
\end{minipage}\hspace{2mm} % 调整间隙
\begin{minipage}{0.25\textwidth}
    \centering
    \small
    \scalebox{0.8}{
    \begin{tabular}{lr}
    \toprule
    \textbf{Method} & \textbf{AVG.} \\ \midrule
    ReFinED & 77.6 \\
    ChatEL(GPT-4) & 80.4 \\
    EntGPT-I(GPT-3.5) & {\underline{84.3}} \\
    \ours & \textbf{86.5} \\ \bottomrule
    \end{tabular}
    }
    \vspace{-1mm}
    \caption{Impact of \ours~on retrieval capabilities assessed through the ED task, presenting average F1 score across nine datasets. Detailed results are in Table in Appendix.}
    \label{table:exp:impact:gr:md2}
\end{minipage}
\end{wrapfigure}

==> tables/temp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{cccccccc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{4}{c}{End-to-End Generation} & \multicolumn{2}{c}{End-to-End Retrieval} \\  \cmidrule{3-8} 
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{HotpotQA} & \multicolumn{2}{c}{2WIKI} & HotpotQA & 2WIKI \\  \cmidrule{3-8} 
\textbf{BackBone} & \textbf{Retriever} & EM & F1 & EM & F1 & Recall@1 & Recall@1 \\  \midrule
 & \multicolumn{1}{c|}{Contriever} & 52.83 & 65.64 & 70.02 & \multicolumn{1}{c|}{74.35} & 73.76 & 68.75 \\
\multirow{-2}{*}{Llama2-7B} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Self} & \cellcolor[HTML]{EFEFEF}\textbf{54.82} & \cellcolor[HTML]{EFEFEF}\textbf{67.93} & \cellcolor[HTML]{EFEFEF}\textbf{75.02} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{78.86}} & \cellcolor[HTML]{EFEFEF}\textbf{75.90} & \cellcolor[HTML]{EFEFEF}\textbf{69.79} \\  \midrule
 & \multicolumn{1}{c|}{Contriever} & 53.72 & 66.46 & 70.92 & \multicolumn{1}{c|}{75.29} & 69.79 & 66.80 \\
\multirow{-2}{*}{Llama3.1-7B} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Self} & \cellcolor[HTML]{EFEFEF}\textbf{55.38} & \cellcolor[HTML]{EFEFEF}\textbf{68.35} & \cellcolor[HTML]{EFEFEF}\textbf{75.88} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{79.60}} & \cellcolor[HTML]{EFEFEF}\textbf{72.55} & \cellcolor[HTML]{EFEFEF}\textbf{68.98} \\  \midrule
 & \multicolumn{1}{c|}{Contriever} & 48.55 & \textbf{61.02} & 68.32 & \multicolumn{1}{c|}{72.66} & 72.41 & 67.70 \\
\multirow{-2}{*}{Qwen2-1.5B} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Self} & \cellcolor[HTML]{EFEFEF}\textbf{48.75} & \cellcolor[HTML]{EFEFEF}60.98 & \cellcolor[HTML]{EFEFEF}\textbf{73.84} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{77.44}} & \cellcolor[HTML]{EFEFEF}\textbf{72.70} & \cellcolor[HTML]{EFEFEF}\textbf{69.27} \\  \midrule
 & \multicolumn{1}{c|}{Contriever} & 53.32 & 66.22 & 70.80 & \multicolumn{1}{c|}{74.86} & 74.15 & 69.01 \\
\multirow{-2}{*}{Qwen2-7B} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Self} & \cellcolor[HTML]{EFEFEF}\textbf{55.12} & \cellcolor[HTML]{EFEFEF}\textbf{67.60} & \cellcolor[HTML]{EFEFEF}\textbf{76.17} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{79.82}} & \cellcolor[HTML]{EFEFEF}\textbf{75.68} & \cellcolor[HTML]{EFEFEF}\textbf{69.96} \\ \bottomrule
\end{tabular}
\end{table}
